Crowding Prediction of In-Situ Metro Passengers Using Smart Card Data

The metro system is playing an increasingly important role in the urban public transit network, transferring a massive human flow across space everyday in the city. In recent years, extensive research studies have been conducted to improve the service quality of metro systems. Among them, crowd management has been a critical issue for both public transport agencies and train operators. In this paper, by utilizing accumulated smart card data, we propose a statistical model to predict in-situ passenger density, i.e., number of on-board passengers between any two neighbouring stations, inside a closed metro system. The proposed model performs two main tasks: i) forecasting time-dependent Origin-Destination (OD) matrix by applying mature statistical models; and ii) estimating the travel time cost required by different parts of the metro network via truncated normal mixture distributions with Expectation-Maximization (EM) algorithm. Based on the prediction results, we are able to provide accurate prediction of in-situ passenger density for a future time point. A case study using real smart card data in Singapore Mass Rapid Transit (MRT) system demonstrate the efficacy and efficiency of our proposed method.

==> Experiment.tex <==
\subsection{Modelling Results}

\subsubsection{Travel time fit}

\begin{figure*}[!htb]
    \centering
    \subfigure[Admiralty to Boon Lay]{
        \includegraphics[width=0.3\textwidth]{Figures/travel_time_pred/single/Admiralty_Boon_Lay.pdf}}
    \subfigure[Jurong East to Woodlands]{
        \includegraphics[width=0.3\textwidth]{Figures/travel_time_pred/single/Jurong_East_Woodlands.pdf} }
    \subfigure[Serangoon to Yio Chu Kang]{
        \includegraphics[width=0.3\textwidth]{Figures/travel_time_pred/single/Serangoon_Yio_Chu_Kang.pdf} }
    \vspace{-0.1in}
    \caption{Fitted travel time of single-route OD pairs}
    \label{fig:travel_time_fit_single}
    \vspace{-0.15in}
\end{figure*}

\begin{figure*}[!htb]
    \centering
    \subfigure[Ang Mo Kio to Harbour Front]{
        \includegraphics[width=0.3\textwidth]{Figures/travel_time_pred/multi/Ang_Mo_Kio_HarbourFront.pdf} }
    \subfigure[Hougang to Kent Ridge]{
        \includegraphics[width=0.3\textwidth]{Figures/travel_time_pred/multi/Hougang_Kent_Ridge.pdf} }
    \subfigure[Yew Tee to City Hall]{
        \includegraphics[width=0.3\textwidth]{Figures/travel_time_pred/multi/Yew_Tee_City_Hall.pdf} }
    \vspace{-0.1in}
    \caption{Fitted travel time of multi-route OD pairs}
    \label{fig:travel_time_fit_multi}
    \vspace{-0.15in}
\end{figure*}

The proposed solution learns the travel time distribution for each OD pair inside the metro system, Fig.~\ref{fig:travel_time_fit_single} and Fig.~\ref{fig:travel_time_fit_multi} report the fitted travel time distribution for sample OD pairs corresponding to single-route OD and multi-route OD respectively. As can be told, for an OD pair with only one candidate route, its corresponding travel time approximates a standalone truncated normal distribution, where we observe only one peak that corresponds to the mean travel time of its route. On the other hand, when an OD pair is linked by multiple candidate routes, multiple peaks are observed on its travel time distribution, with each peak corresponds to the mean travel time of one of the candidate routes, and height of peak being proportional to the route preference probability. Also, we note that for certain multi-route OD pairs, such as OD pair $<x, x>$, only a single peak in its travel time distribution is spotted. This is consistent with our daily experience that people do not necessary travel every candidate route of an OD pair, only those routes that are more convenient to travel are frequently used. 
%In order to assess the goodness of travel time estimation, the average log-likelihood between each posterior estimate and the actual travel time observation is computed as well in Table~\ref{tab:single-path-time-prediction-result} and Table~\ref{tab:multi-path-time-prediction-result}.

% \begin{table}[t!]
% \caption{Travel Time Prediction Log-likelihood}
% \centering
% \label{tab:single-path-time-prediction-result}
% \begin{tabular}{|l||l|l||l|l|}
% \hline
%  &\multicolumn{2}{c|}{Singapore}&\multicolumn{2}{c|}{Taipei}\\
% \cline{2-5}
%  & Morning Peak & Evening Peak & Morning Peak & Evening Peak\\
% \hline\hline
% FLOW & 0.130 & XX & XX & XX\\
% TripDecoder & 0.126 & 0.120 & XX & XX\\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[t!]
% \caption{Multi-path Travel Time Prediction Log-likelihood}
% \centering
% \label{tab:multi-path-time-prediction-result}
% \begin{tabular}{|l||l|l||l|l|}
% \hline
%  &\multicolumn{2}{c|}{Singapore}&\multicolumn{2}{c|}{Taipei}\\
% \cline{2-5}
%  & Morning Peak & Evening Peak & Morning Peak & Evening Peak\\
% \hline\hline
% FLOW & 0.100 & XX & XX & XX\\
% TripDecoder & 0.091 & 0.077 & XX & XX\\
% \hline
% \end{tabular}
% \end{table}

% The higher log-likelihood belongs to the proposed solution, which indicates its higher predictive power.


\subsubsection{Alight rate fit}
As EZ-link card records alight station and alight date time for each ride, the actual alight rate can be easily calculated, which can be used as ground truth to measure the accuracy of the proposed solution. We predict the alight based on Equation~\eqref{eq:tap_out_flow}. Fig.~\ref{fig:alight_rate} reports prediction of alight rate for sample MRT stations. In each sub-graph, the actual alight rate, historical average rate and our prediction are reported. The graphs show that the proposed solution is able to render accurate prediction of alight rate, which is more accurate than using historical average alight rate. Based on the graphs, we can see that for MRT stations located in residential area, such as Ang Mo Kio and Bukit Gombak station, the alight rate peaks show up at evening peak hour, when people knock off from office and take MRT to go home. On the other hand, for MRT stations located in CBD area, the alight rate peak shows up at morning peak hour, when people take MRT from home to the office in the morning.

\begin{figure*}[!htb]
    \centering
    \subfigure[Ang Mo Kio]{
        \includegraphics[width=0.3\textwidth]{Figures/alight_rate_pred/Ang_Mo_Kio.pdf} }
    \subfigure[Bukit Gombak]{
        \includegraphics[width=0.3\textwidth]{Figures/alight_rate_pred/Bukit_Gombak.pdf} }
    \subfigure[Raffles Place]{
        \includegraphics[width=0.3\textwidth]{Figures/alight_rate_pred/Raffles_Place.pdf} }
    \vspace{-0.1in}
    \caption{Alight rate prediction}
    \label{fig:alight_rate}
    \vspace{-0.15in}
\end{figure*}

% \begin{figure*}[t!]
% \centering
% \includegraphics[width=16cm]{Figures/tap_out_pred/alight_rate_heatmap.pdf}
% \caption{Alight Rate of East-West Line Stations}
% \label{fig:alight_rate_heatmap}
% \end{figure*}

% From the heat map in Figure~\ref{fig:alight_rate_heatmap}, some interesting insights can be extracted. On one hand, from 8:30am to 9:30am, both Tanjong Pagar and Raffles Place have very high alight rate, this is probably because there are many office buildings nearby the two stations, in the morning people work there would tap out at the stations and go to their office. On the other hand, we also spot high alight rate at a few station from 6:30pm to 7:30pm, these stations are usually surrounded by residence areas, and often are equipped with facilities like community center and shopping malls. After work, people living in the neighbor would take train and alight there, people stay nearby may also make transfer at these stations, thus that they can have dinner there with their family or friends, or just go grocery shopping. Station of this kind include Boon Lay, Clementi, Bedok, Tampines and Pasir Ris. We also notice that there is another type of stations, they have relatively high alight rate almost across the whole day, it seems that at different time, there are people who would like to visit these stations for certain purposes, some of this kind of station are Jurong East, City Hall and Bugis, it turns out that these stations are all located with big shopping malls and lots of restaurants, they also serve as the interchange stations for differnt MRT lines, which explains why they can attract high human flows at different time of the day.

% \begin{comment}
% \begin{figure*}[!htb]
%     \centering
%     \subfigure[Buona Vista]{
%         \includegraphics[width=0.3\textwidth]{Figures/tap_out_pred/Buona_Vista.jpg} }
%     \subfigure[Newton]{
%         \includegraphics[width=0.3\textwidth]{Figures/tap_out_pred/Newton.jpg} }
%     \subfigure[Paya Lebar]{
%         \includegraphics[width=0.3\textwidth]{Figures/tap_out_pred/Paya_Lebar.jpg} }
%     \vspace{-0.1in}
%     \caption{Tap out flow prediction}
%     \label{fig:tap_out_flow}
%     \vspace{-0.15in}
% \end{figure*}
% \end{comment}

\subsubsection{Passenger flow inside MRT network}

\begin{figure*}[!htb]
    \centering
    \subfigure[8:30 am]{
        \includegraphics[width=0.45\textwidth]{Figures/system_flow_pred/8_30.pdf}}
    \subfigure[6:30 pm]{
        \includegraphics[width=0.45\textwidth]{Figures/system_flow_pred/18_30.pdf}}
    \vspace{-0.1in}
    \caption{System passenger flow snapshot}
    \label{fig:network_passenger_load}
    \vspace{-0.15in}
\end{figure*}

Fig.~\ref{fig:network_passenger_load} provide snapshots of real time passenger flow of metro network at time XX and time XX, which could possibly reflect the passenger flow during morning peak hour and evening peak hour respectively. Notice that passenger flow are bi-directional, here we only show passenger flow on one direction. On sub-figure XX, we can easily tell that...
